Fairguard: Harness Logic-based Fairness Rules in Smart Cities

Smart cities operate on computational predictive frameworks that collect, aggregate, and utilize data from large-scale sensor networks. However, these frameworks are prone to multiple sources of data and algorithmic bias, which often lead to unfair prediction results. In this work, we first demonstrate that bias persists at a micro-level both temporally and spatially by studying real city data from Chattanooga, TN. To alleviate the issue of such bias, we introduce Fairguard, a micro-level temporal logic-based approach for fair smart city policy adjustment and generation in complex temporal-spatial domains. The Fairguard framework consists of two phases: first, we develop a static generator that is able to reduce data bias based on temporal logic conditions by minimizing correlations between selected attributes. Then, to ensure fairness in predictive algorithms, we design a dynamic component to regulate prediction results and generate future fair predictions by harnessing logic rules. Evaluations show that logic-enabled static Fairguard can effectively reduce the biased correlations while dynamic Fairguard can guarantee fairness on protected groups at run-time with minimal impact on overall performance.

==> 8_not_needed.tex <==
% We should delete things about SC.
% The SC (equation \ref{eq:2}) of variables X and Y, according to Hotelling and Pabst (Citation needed here), is displayed in the equation below with \begin{math}d_i\end{math} being the difference between the ranks of the ith element in X and Y.

% \begin{equation} \label{eq:2}
%     SC_{XY} = 1 - \frac{6\sum(d_{i}^2)}{n^3 - n}
% \end{equation}

% Hauke and Kossowski (Citation needed here) suggested that PC evaluates linear relationships, whereas SC, as a nonparametric rank statistic, describes how well any monotonic function explains the relationship between two variables. Since some PAs in a given timeframe, with respect to the scaled bike demands, manifest linear relationships (Figure 3: Put a figure of a linear PA wpt BD), whereas some others manifest non-linearly (Figure 4: Put a figure of a non-linear PA wpt BD), we chose both PC and SC for the feedback requirements.

==> Note.tex <==
% For the research tracks, submissions are limited to 8 content pages, which should include all figures and tables. In addition, you can include up to 2 pages of additional supplementary material, plus additional pages for references, until completing a maximum of 12 pages. The total count of pages of your submission must not exceed 12 pages. Papers must be formatted according to the instructions below, and those not complying to the page limits or not following the formatting guidelines will be desk-rejected. Authors will also be asked to confirm their length compliance during paper submission.

% Important dates
% Abstract submission: Thursday, October 6, 2022. This is compulsory for all papers.
% Full papers submission: Thursday, October 13, 2022
% Rebuttal: Thursday, December 22, 2022
% Notification: Wednesday, January 25, 2023
% All submission deadlines are end-of-day in the Anywhere on Earth (AoE) time zone.
